RAGTurk: Best Practices for Retrieval Augmented Generation in Turkish

Retrieval-Augmented Generation (RAG) enhances LLM factuality, yet design guidance remains English-centric, limiting insights for morphologically rich languages like Turkish. We address this by constructing a comprehensive Turkish RAG dataset derived from Turkish Wikipedia and CulturaX, comprising question-answer pairs and relevant passage chunks. We benchmark seven stages of the RAG pipeline, from query transformation and reranking to answer refinement, without task-specific fine-tuning. Our results show that complex methods like HyDE maximize accuracy (85%) that is considerably higher than the baseline (78.70%). Also a Pareto-optimal configuration using Cross-encoder Reranking and Context Augmentation achieves comparable performance (84.60%) with much lower cost. We further demonstrate that over-stacking generative modules can degrade performance by distorting morphological cues, whereas simple query clarification with robust reranking offers an effective solution.

==> main <==
@inproceedings{umutlu-etal-2025-evaluating,
    title = "Evaluating the Quality of Benchmark Datasets for Low-Resource Languages: A Case Study on {T}urkish",
    author = "Umutlu, Elif Ecem  and
      Cengiz, Ayse Aysu  and
      Sever, Ahmet Kaan  and
      Erdem, Seyma  and
      Aytan, Burak  and
      Tufan, Busra  and
      Topraksoy, Abdullah  and
      Dar{\i}c{\i}, Esra  and
      Toraman, Cagri",
    editor = "Arviv, Ofir  and
      Clinciu, Miruna  and
      Dhole, Kaustubh  and
      Dror, Rotem  and
      Gehrmann, Sebastian  and
      Habba, Eliya  and
      Itzhak, Itay  and
      Mille, Simon  and
      Perlitz, Yotam  and
      Santus, Enrico  and
      Sedoc, Jo{\~a}o  and
      Shmueli Scheuer, Michal  and
      Stanovsky, Gabriel  and
      Tafjord, Oyvind",
    booktitle = "Proceedings of the Fourth Workshop on Generation, Evaluation and Metrics (GEM{\texttwosuperior})",
    month = jul,
    year = "2025",
    address = "Vienna, Austria and virtual meeting",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2025.gem-1.41/",
    pages = "471--487",
    ISBN = "979-8-89176-261-9",
    abstract = "The reliance on translated or adapted datasets from English or multilingual resources introduces challenges regarding linguistic and cultural suitability. This study addresses the need for robust and culturally appropriate benchmarks by evaluating the quality of 17 commonly used Turkish benchmark datasets. Using a comprehensive framework that assesses six criteria, both human and LLM-judge annotators provide detailed evaluations to identify dataset strengths and shortcomings.Our results reveal that 70{\\%} of the benchmark datasets fail to meet our heuristic quality standards. The correctness of the usage of technical terms is the strongest criterion, but 85{\\%} of the criteria are not satisfied in the examined datasets. Although LLM judges demonstrate potential, they are less effective than human annotators, particularly in understanding cultural common sense knowledge and interpreting fluent, unambiguous text. GPT-4o has stronger labeling capabilities for grammatical and technical tasks, while Llama3.3-70B excels at correctness and cultural knowledge evaluation. Our findings emphasize the urgent need for more rigorous quality control in creating and adapting datasets for low-resource languages."
}

@article{hakkani2002statistical,
  title={Statistical morphological disambiguation for agglutinative languages},
  author={Hakkani-T{\"u}r, Dilek Z and Oflazer, Kemal and T{\"u}r, G{\"o}khan},
  journal={Computers and the Humanities},
  volume={36},
  number={4},
  pages={381--410},
  year={2002},
  publisher={Springer}
}

@article{oflazer2014turkish,
  title={{Turkish} and its Challenges for Language Processing},
  author={Oflazer, Kemal},
  journal={Language resources and evaluation},
  volume={48},
  number={4},
  pages={639--653},
  year={2014},
  publisher={Springer}
}

@article{toraman2026turkbench,
  title={TurkBench: A Benchmark for Evaluating Turkish Large Language Models},
  author={Toraman, Çağrı and Sever, Ahmet Kaan and Cengiz, Ayse Aysu and Arslan, Elif Ecem and Sevinç, Görkem and Birdal, Mete Mert and Güldemir, Yusuf Faruk and Kanburoğlu, Ali Buğra and Felekoğlu, Sezen and Gürlek, Osman and Kantar, Sarp and Kütük, Birsen Şahin and Tufan, Büşra and Genç, Elif and Coşkun, Serkan and Demir, Gupse Ekin and Arayıcı, Muhammed Emin and Dursun, Olgun and Gungor, Onur and Üsküdarlı, Susan and Topraksoy, Abdullah and Darıcı, Esra},
  journal={arXiv preprint arXiv:2601.07020},
  year={2026}
}


@book{Aho:72,
    author  = {Alfred V. Aho and Jeffrey D. Ullman},
    title   = {The Theory of Parsing, Translation and Compiling},
    year    = "1972",
    volume  = "1",
    publisher = {Prentice-Hall},
    address = {Englewood Cliffs, NJ}
}

@book{APA:83,
    author  = {{American Psychological Association}},
    title   = {Publications Manual},
    year    = "1983",
    publisher = {American Psychological Association},
    address = {Washington, DC}
}

@article{Chandra:81,
	author = {Ashok K. Chandra and Dexter C. Kozen and Larry J. Stockmeyer},
	year = "1981",
	title = {Alternation},
	journal = {Journal of the Association for Computing Machinery},
	volume = "28",
	number = "1",
	pages = "114--133",
	doi = "10.1145/322234.322243",
}

@inproceedings{andrew2007scalable,
  title={Scalable training of {L1}-regularized log-linear models},
  author={Andrew, Galen and Gao, Jianfeng},
  booktitle={Proceedings of the 24th International Conference on Machine Learning},
  pages={33--40},
  year={2007},
}

@book{Gusfield:97,
    author  = {Dan Gusfield},
    title   = {Algorithms on Strings, Trees and Sequences},
    year    = "1997",
    publisher = {Cambridge University Press},
    address = {Cambridge, UK}
}

@article{rasooli-tetrault-2015,
    author    = {Mohammad Sadegh Rasooli and Joel R. Tetreault},
    title     = {Yara Parser: {A} Fast and Accurate Dependency Parser},
    journal   = {Computing Research Repository},
    volume    = {arXiv:1503.06733},
    year      = {2015},
    url       = {http://arxiv.org/abs/1503.06733},
    note    = {version 2}
}

@article{Ando2005,
	Acmid = {1194905},
	Author = {Ando, Rie Kubota and Zhang, Tong},
	Issn = {1532-4435},
	Issue_Date = {12/1/2005},
	Journal = {Journal of Machine Learning Research},
	Month = dec,
	Numpages = {37},
	Pages = {1817--1853},
	Publisher = {JMLR.org},
	Title = {A Framework for Learning Predictive Structures from Multiple Tasks and Unlabeled Data},
	Volume = {6},
	Year = {2005}
}

@inproceedings{nguyen-etal-2024-culturax,
    title = "{C}ultura{X}: A Cleaned, Enormous, and Multilingual Dataset for Large Language Models in 167 Languages",
    author = "Nguyen, Thuat  and
      Nguyen, Chien Van  and
      Lai, Viet Dac  and
      Man, Hieu  and
      Ngo, Nghia Trung  and
      Dernoncourt, Franck  and
      Rossi, Ryan A.  and
      Nguyen, Thien Huu",
    editor = "Calzolari, Nicoletta  and
      Kan, Min-Yen  and
      Hoste, Veronique  and
      Lenci, Alessandro  and
      Sakti, Sakriani  and
      Xue, Nianwen",
    booktitle = "Proceedings of the 2024 Joint International Conference on Computational Linguistics, Language Resources and Evaluation (LREC-COLING 2024)",
    month = may,
    year = "2024",
    address = "Torino, Italia",
    publisher = "ELRA and ICCL",
    url = "https://aclanthology.org/2024.lrec-main.377/",
    pages = "4226--4237"
}

@article{lewis2020rag,
  title         = {Retrieval-Augmented Generation for Knowledge-Intensive {NLP} Tasks},
  author        = {Lewis, Patrick and Perez, Ethan and Piktus, Aleksandra and Petroni, Fabio and Karpukhin, Vladimir and Goyal, Naman and K{\"u}ttler, Heinrich and Lewis, Mike and Yih, Wen-tau and Rockt{\"a}schel, Tim and Riedel, Sebastian and Kiela, Douwe},
  journal       = {arXiv preprint arXiv:2005.11401},
  year          = {2020},
  url           = {https://arxiv.org/abs/2005.11401}
}

@inproceedings{karpukhin2020dpr,
  title         = {Dense Passage Retrieval for Open-Domain Question Answering},
  author        = {Karpukhin, Vladimir and Oguz, Barlas and Min, Sewon and Lewis, Patrick and Wu, Ledell and Edunov, Sergey and Chen, Danqi and Yih, Wen-tau},
  booktitle     = {Proceedings of EMNLP},
  year          = {2020},
  url           = {https://arxiv.org/abs/2004.04906}
}

@article{nogueira2019bert_rerank,
  title         = {Passage Re-ranking with {BERT}},
  author        = {Nogueira, Rodrigo and Cho, Kyunghyun},
  journal       = {arXiv preprint arXiv:1901.04085},
  year          = {2019},
  url           = {https://arxiv.org/abs/1901.04085}
}

@inproceedings{cormack2009rrf,
  title         = {Reciprocal Rank Fusion outperforms {Condorcet} and Individual Rank Learning Methods},
  author        = {Cormack, Gordon V. and Clarke, Charles L. A. and B{\"u}ttcher, Stefan},
  booktitle     = {Proceedings of SIGIR},
  year          = {2009},
  pages         = {758--759},
  doi           = {10.1145/1571941.1572114},
  url           = {https://dl.acm.org/doi/10.1145/1571941.1572114}
}

@article{rackauckas2024ragfusion,
  title         = {{RAG}-Fusion: a New Take on Retrieval-Augmented Generation},
  author        = {Rackauckas, Zackary},
  journal       = {arXiv preprint arXiv:2402.03367},
  year          = {2024},
  url           = {https://arxiv.org/abs/2402.03367}
}

@inproceedings{wang2023query2doc,
  title         = {Query2doc: Query Expansion with Large Language Models},
  author        = {Wang, Liang and Yang, Nan and Wei, Furu},
  booktitle     = {Proceedings of EMNLP},
  year          = {2023},
  url           = {https://aclanthology.org/2023.emnlp-main.585/}
}

@inproceedings{mao2021gar,
  title         = {Generation-Augmented Retrieval for Open-Domain Question Answering},
  author        = {Mao, Yuning and He, Pengcheng and Liu, Xiaodong and Shen, Yelong and Gao, Jianfeng and Han, Jiawei and Chen, Weizhu},
  booktitle     = {Proceedings of ACL},
  year          = {2021},
  url           = {https://aclanthology.org/2021.acl-long.316/}
}

@article{nogueira2019doc2query,
  title         = {Document Expansion by Query Prediction},
  author        = {Nogueira, Rodrigo and Yang, Wei and Lin, Jimmy and Cho, Kyunghyun},
  journal       = {arXiv preprint arXiv:1904.08375},
  year          = {2019},
  url           = {https://arxiv.org/abs/1904.08375}
}

@article{gao2023hyde,
  title         = {Precise Zero-Shot Dense Retrieval without Relevance Labels},
  author        = {Gao, Luyu and Ma, Xueguang and Lin, Jimmy and Callan, Jamie},
  journal       = {arXiv preprint arXiv:2212.10496},
  year          = {2022},
  url           = {https://arxiv.org/abs/2212.10496}
}

@article{vake2025hype,
  title         = {Bridging the Question--Answer Gap in Retrieval-Augmented Generation: {Hypothetical Prompt Embeddings}},
  author        = {Vake, Domen and Vi{\v{c}}i{\v{c}}, Jernej and To{\v{s}}i{\v{c}}, Aleksandar},
  journal       = {IEEE Access},
  year          = {2025},
  doi           = {10.1109/ACCESS.2025.3589499},
  url           = {https://ieeexplore.ieee.org/document/11080443}
}

@article{liu2025lgmgc,
  title         = {Passage Segmentation of Documents for Extractive Question Answering},
  author        = {Liu, Zuhong and Simon, Charles-Elie and Caspani, Fabien},
  journal       = {arXiv preprint arXiv:2501.09940},
  year          = {2025},
  url           = {https://arxiv.org/abs/2501.09940}
}

@article{zheng2024stepback,
  title         = {Take a Step Back: Evoking Reasoning via Abstraction in Large Language Models},
  author        = {Zheng, Huaixiu Steven and Mishra, Swaroop and Chen, Xinyun and Cheng, Heng-Tze and Chi, Ed H. and Le, Quoc V. and Zhou, Denny},
  journal       = {arXiv preprint arXiv:2310.06117},
  year          = {2023},
  note          = {ICLR 2024},
  url           = {https://arxiv.org/abs/2310.06117}
}

@article{liu2024lostmiddle,
  title         = {Lost in the Middle: How Language Models Use Long Contexts},
  author        = {Liu, Nelson F. and Lin, Kevin and Hewitt, John and Paranjape, Ashwin and Bevilacqua, Michele and Petroni, Fabio and Liang, Percy},
  journal       = {Transactions of the Association for Computational Linguistics},
  year          = {2024},
  url           = {https://aclanthology.org/2024.tacl-1.9/}
}

@article{jiang2023llmlingua,
  title         = {{LLMLingua}: Compressing Prompts for Accelerated Inference of Large Language Models},
  author        = {Jiang, Huiqiang and Wu, Qianhui and Lin, Chin-Yew and Yang, Yuqing and Qiu, Lili},
  journal       = {arXiv preprint arXiv:2310.05736},
  year          = {2023},
  url           = {https://arxiv.org/abs/2310.05736}
}

@inproceedings{li2023selectivecontext,
  title         = {Compressing Context to Enhance Inference Efficiency of Large Language Models},
  author        = {Li, Yucheng and Dong, Bo and Lin, Chenghua and Guerin, Frank},
  booktitle     = {Proceedings of EMNLP},
  year          = {2023},
  url           = {https://arxiv.org/abs/2310.06201}
}

@article{madaan2023selfrefine,
  title         = {Self-Refine: Iterative Refinement with Self-Feedback},
  author        = {Madaan, Aman and Tandon, Niket and Gupta, Prakhar and Hallinan, Skyler and Gao, Luyu and Wiegreffe, Sarah and Alon, Uri and Dziri, Nouha and Prabhumoye, Shrimai and Yang, Yiming and Gupta, Shashank and Majumder, Bodhisattwa Prasad and Hermann, Katherine and Welleck, Sean and Yazdanbakhsh, Amir and Clark, Peter},
  journal       = {arXiv preprint arXiv:2303.17651},
  year          = {2023},
  url           = {https://arxiv.org/abs/2303.17651}
}

@article{shinn2023reflexion,
  title         = {Reflexion: Language Agents with Verbal Reinforcement Learning},
  author        = {Shinn, Noah and Cassano, Federico and Berman, Edward and Gopinath, Ashwin and Narasimhan, Karthik and Yao, Shunyu},
  journal       = {arXiv preprint arXiv:2303.11366},
  year          = {2023},
  note          = {NeurIPS 2023},
  url           = {https://arxiv.org/abs/2303.11366}
}

@article{kartal2025ragsmith,
  title         = {{RAGSmith}: A Framework for Finding the Optimal Composition of Retrieval-Augmented Generation Methods Across Datasets},
  author        = {Kartal, Muhammed Yusuf and K{\"o}se, Suha Kagan and Sevin{\c{c}}, Korhan and Aktas, Burak},
  journal       = {arXiv preprint arXiv:2511.01386},
  year          = {2025},
  doi           = {10.48550/arXiv.2511.01386},
  url           = {https://arxiv.org/abs/2511.01386}
}

@misc{gupta2024rag_survey,
  title         = {A Comprehensive Survey of Retrieval-Augmented Generation ({RAG}): Evolution, Current Landscape and Future Directions},
  author        = {Gupta, Shailja and Ranjan, Rajesh and Singh, Surya Narayan},
  year          = {2024},
  howpublished  = {arXiv preprint},
  eprint        = {2410.12837},
  archivePrefix = {arXiv},
  url           = {https://arxiv.org/abs/2410.12837}
}


@misc{zhao2024rag_aigc_survey,
  title         = {Retrieval-Augmented Generation for {AI}-Generated Content: A Survey},
  author        = {Zhao, Penghao and Zhang, Hailin and Yu, Qinhan and Wang, Zhengren and Geng, Yunteng and Fu, Fangcheng and Yang, Ling and Zhang, Wentao and Jiang, Jie and Cui, Bin},
  year          = {2024},
  howpublished  = {arXiv preprint},
  eprint        = {2402.19473},
  archivePrefix = {arXiv},
  primaryClass  = {cs.CV},
  doi           = {10.48550/arXiv.2402.19473},
  url           = {https://arxiv.org/abs/2402.19473}
}

@misc{liu2025ragSurvey,
  title        = {Retrieval-Augmented Generation: {A} Survey of Methodologies, Techniques, Applications, and Future Directions},
  author       = {Liu, Charles Z. and Abayakoon, Imani and Khadeer Hussain, Farookh},
  year         = {2025},
  month        = nov,
  howpublished = {Preprint},
  doi          = {10.31224/5781},
  url          = {https://doi.org/10.31224/5781}
}

@inproceedings{lin2021pyserini,
  title     = {{Pyserini}: A {Python} Toolkit for Reproducible Information Retrieval Research with Sparse and Dense Representations},
  author    = {Lin, Jimmy and Ma, Xueguang and Lin, Sheng-Chieh and Yang, Jheng-Hong and Pradeep, Ronak and Nogueira, Rodrigo},
  booktitle = {Proceedings of the 44th International ACM SIGIR Conference on Research and Development in Information Retrieval (SIGIR '21)},
  year      = {2021},
  month     = jul,
  address   = {Virtual Event, Canada},
  publisher = {ACM},
  pages     = {2356--2362},
  doi       = {10.1145/3404835.3463238},
  url       = {https://dl.acm.org/doi/10.1145/3404835.3463238}
}


@inproceedings{khattab2020colbert,
  title     = {{ColBERT}: Efficient and Effective Passage Search via Contextualized Late Interaction over {BERT}},
  author    = {Khattab, Omar and Zaharia, Matei},
  booktitle = {Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval (SIGIR '20)},
  year      = {2020},
  publisher = {ACM},
  pages     = {39--48},
  doi       = {10.1145/3397271.3401075},
  url       = {https://dl.acm.org/doi/10.1145/3397271.3401075}
}


@misc{li2025qeSurvey,
  title         = {Query Expansion in the Age of Pre-trained and Large Language Models: A Comprehensive Survey},
  author        = {Li, Minghan and Lv, Xinxuan and Zou, Junjie and Chen, Tongna and Zhang, Chao and An, Suchao and Nie, Ercong and Zhou, Guodong},
  year          = {2025},
  howpublished  = {arXiv preprint},
  eprint        = {2509.07794},
  archivePrefix = {arXiv},
  doi           = {10.48550/arXiv.2509.07794},
  url           = {https://arxiv.org/abs/2509.07794}
}


@inproceedings{tao-etal-2025-treerag,
  title     = {{TreeRAG}: Unleashing the Power of Hierarchical Storage for Enhanced Knowledge Retrieval in Long Documents},
  author    = {Tao, Wenyu and Xing, Xiaofen and Chen, Yirong and Huang, Linyi and Xu, Xiangmin},
  booktitle = {Findings of the Association for Computational Linguistics: ACL 2025},
  year      = {2025},
  month     = jul,
  address   = {Vienna, Austria},
  publisher = {Association for Computational Linguistics},
  pages     = {356--371},
  url       = {https://aclanthology.org/2025.findings-acl.20/}
}

@inproceedings{asai2024selfrag,
  title     = {Self-{RAG}: Learning to Retrieve, Generate, and Critique through Self-Reflection},
  author    = {Asai, Akari and Wu, Zeqiu and Wang, Yizhong and Sil, Avirup and Hajishirzi, Hannaneh},
  booktitle = {International Conference on Learning Representations (ICLR)},
  year      = {2024},
  url       = {https://openreview.net/forum?id=hSyW5go0v8},
  note      = {Oral}
}


@inproceedings{jiang-etal-2023-active,
  title     = {Active Retrieval Augmented Generation},
  author    = {Jiang, Zhengbao and Xu, Frank F. and Gao, Luyu and Sun, Zhiqing and Liu, Qian and Dwivedi-Yu, Jane and Yang, Yiming and Callan, Jamie and Neubig, Graham},
  booktitle = {Proceedings of the 2023 Conference on Empirical Methods in Natural Language Processing},
  year      = {2023},
  month     = dec,
  address   = {Singapore},
  publisher = {Association for Computational Linguistics},
  pages     = {7969--7992},
  doi       = {10.18653/v1/2023.emnlp-main.495},
  url       = {https://aclanthology.org/2023.emnlp-main.495/}
}


@misc{yu2024evaluationrag,
  title         = {Evaluation of Retrieval-Augmented Generation: {A} Survey},
  author        = {Yu, Hao and Gan, Aoran and Zhang, Kai and Tong, Shiwei and Liu, Qi and Liu, Zhaofeng},
  year          = {2024},
  howpublished  = {arXiv preprint},
  eprint        = {2405.07437},
  archivePrefix = {arXiv},
  primaryClass  = {cs.CL},
  doi           = {10.48550/arXiv.2405.07437},
  url           = {https://arxiv.org/abs/2405.07437}
}


@inproceedings{es-etal-2024-ragas,
  title     = {{RAGAs}: Automated Evaluation of Retrieval Augmented Generation},
  author    = {Es, Shahul and James, Jithin and Espinosa-Anke, Luis and Schockaert, Steven},
  booktitle = {Proceedings of the 18th Conference of the European Chapter of the Association for Computational Linguistics: System Demonstrations},
  year      = {2024},
  publisher = {Association for Computational Linguistics},
  url       = {https://aclanthology.org/2024.eacl-demo.16/}
}

@article{bikmaz2025bridging,
  title   = {Bridging the Language Gap in {RAG}: A Case Study on {Turkish} Retrieval and Generation},
  author  = {Bikmaz, Erdo{\u{g}}an and Briman, Mohammed and Arslan, Serdar},
  journal = {Researcher},
  volume  = {5},
  number  = {1},
  pages   = {38--49},
  year    = {2025},
  url     = {https://dergipark.org.tr/en/pub/researcher/article/1699017}
}


@misc{simsek2025turkishculturalrag,
  title        = {Retrieval-Augmented Generation versus Fine-tuning for {Turkish} Cultural Question Answering: A Comprehensive Evaluation and Analysis},
  author       = {Simsek, Murat},
  year         = {2025},
  howpublished = {Research Square preprint},
  doi          = {10.21203/rs.3.rs-7217024/v1},
  url          = {https://sciety.org/articles/activity/10.21203/rs.3.rs-7217024/v1}
}

@misc{ezerceli2025turkembed4retrieval,
  title         = {{TurkEmbed4Retrieval}: {Turkish} Embedding Model for Retrieval Task},
  author        = {Ezerceli, {\"O}zay and G{\"u}m{\"u}{\c{s}}\c{c}eki\c{c}ci, Gizem and Erko{\c{c}}, Tu{\u{g}}ba and {\"O}zen{\c{c}}, Berke},
  year          = {2025},
  howpublished  = {arXiv preprint},
  eprint        = {2511.07595},
  archivePrefix = {arXiv},
  url           = {https://arxiv.org/abs/2511.07595}
}


@misc{tas2025turklettucedetect,
  title         = {Turk-LettuceDetect: A Hallucination Detection Models for {Turkish} {RAG} Applications},
  author        = {Ta{\c{s}}, Selva and El Huseyni, Mahmut and Ezerceli, {\"O}zay and Bayraktar, Reyhan and Terzio{\u{g}}lu, Fatma Bet{\"u}l},
  year          = {2025},
  howpublished  = {arXiv preprint},
  eprint        = {2509.17671},
  archivePrefix = {arXiv},
  doi           = {10.48550/arXiv.2509.17671},
  url           = {https://arxiv.org/abs/2509.17671}
}


@misc{kim2024autorag,
  title         = {{AutoRAG}: Automated Framework for Optimization of Retrieval Augmented Generation Pipeline},
  author        = {Kim, Dongkyu and Kim, Byoungwook and Han, Donggeon and Eibich, Matou{\v{s}}},
  year          = {2024},
  howpublished  = {arXiv preprint},
  eprint        = {2410.20878},
  archivePrefix = {arXiv},
  doi           = {10.48550/arXiv.2410.20878},
  url           = {https://arxiv.org/abs/2410.20878}
}


@inproceedings{khattab2024dspy,
  title     = {{DSP}y: Compiling Declarative Language Model Calls into State-of-the-Art Pipelines},
  author    = {Khattab, Omar and Singhvi, Arnav and Maheshwari, Paridhi and Zhang, Zhiyuan and Santhanam, Keshav and Vardhamanan, Sri and Haq, Saiful and Sharma, Ashutosh and Joshi, Thomas T. and Moazam, Hanna and Miller, Heather and Zaharia, Matei and Potts, Christopher},
  booktitle = {The Twelfth International Conference on Learning Representations (ICLR 2024)},
  year      = {2024},
  url       = {https://openreview.net/forum?id=sY5N0zY5Od}
}


@misc{edge2024graphrag,
  title         = {From Local to Global: A Graph {RAG} Approach to Query-Focused Summarization},
  author        = {Edge, Darren and Trinh, Ha and Cheng, Newman and Bradley, Joshua and Chao, Alex and Mody, Apurva and Truitt, Steven and Metropolitansky, Dasha and Ness, Robert Osazuwa and Larson, Jonathan},
  year          = {2024},
  howpublished  = {arXiv preprint},
  eprint        = {2404.16130},
  archivePrefix = {arXiv},
  url           = {https://arxiv.org/abs/2404.16130}
}


@misc{turkbench,
  title = {TurkBench Leaderboard},
  howpublished = {\url{https://huggingface.co/spaces/TurkBench/TurkBench}},
  year = {2024}
}

@misc{openai2025gptoss,
  title         = {gpt-oss-120b \& gpt-oss-20b Model Card},
  author        = {{OpenAI}},
  year          = {2025},
  eprint        = {2508.10925},
  archivePrefix = {arXiv},
  primaryClass  = {cs.CL},
  url           = {https://arxiv.org/abs/2508.10925},
  note          = {\url{https://openai.com/research/gpt-oss-model-card/}}
}

@misc{google2025gemini25models,
  title        = {Gemini API: Model information},
  author       = {{Google}},
  year         = {2025},
  url          = {https://ai.google.dev/gemini-api/docs/models},
  note         = {Accessed: 2025-12-24}
}

@book{holland1975adaptation,
  title     = {Adaptation in Natural and Artificial Systems},
  author    = {Holland, John H.},
  year      = {1975},
  publisher = {University of Michigan Press},
  address   = {Ann Arbor, MI}
}

@book{goldberg1989genetic,
  title     = {Genetic Algorithms in Search, Optimization, and Machine Learning},
  author    = {Goldberg, David E.},
  year      = {1989},
  publisher = {Addison-Wesley},
  address   = {Reading, MA}
}

@misc{gao2020pile,
  title        = {The {P}ile: An 800GB Dataset of Diverse Text for Language Modeling},
  author       = {Gao, Leo and Biderman, Stella and Black, Sid and Golding, Laurence and Hoppe, Travis and Foster, Charles and Phang, Jason and He, Horace and Thite, Anish and Nabeshima, Noa and Presser, Shawn and Leahy, Connor},
  year         = {2020},
  howpublished = {arXiv:2101.00027},
  doi          = {10.48550/arXiv.2101.00027},
  url          = {https://arxiv.org/abs/2101.00027}
}

@misc{biderman2022datasheetpile,
  title        = {Datasheet for the {P}ile},
  author       = {Biderman, Stella and Bicheno, Kieran and Gao, Leo},
  year         = {2022},
  howpublished = {arXiv:2201.07311},
  doi          = {10.48550/arXiv.2201.07311},
  url          = {https://arxiv.org/abs/2201.07311}
}

@inproceedings{soldaini-etal-2024-dolma,
  title     = {{Dolma}: an Open Corpus of Three Trillion Tokens for Language Model Pretraining Research},
  author    = {Soldaini, Luca and others},
  booktitle = {Proceedings of the 62nd Annual Meeting of the Association for Computational Linguistics (ACL)},
  year      = {2024},
  url       = {https://aclanthology.org/2024.acl-long.9/}
}

@misc{weber2024redpajama,
  title        = {{RedPajama}: an Open Dataset for Training Large Language Models},
  author       = {Weber, Maurice and Fu, Daniel and Anthony, Quentin and Oren, Yonatan and Adams, Shane and Alexandrov, Anton and Lyu, Xiaozhong and Nguyen, Huu and Yao, Xiaozhe and Adams, Virginia and Athiwaratkun, Ben and Chalamala, Rahul and Chen, Kezhen and Ryabinin, Max and Dao, Tri and Liang, Percy and R{\'e}, Christopher and Rish, Irina and Zhang, Ce},
  year         = {2024},
  howpublished = {arXiv:2411.12372},
  doi          = {10.48550/arXiv.2411.12372},
  url          = {https://arxiv.org/abs/2411.12372}
}

@inproceedings{wenzek-etal-2020-ccnet,
  title     = {{CCN}et: Extracting High Quality Monolingual Datasets from Web Crawl Data},
  author    = {Wenzek, Guillaume and Lachaux, Marie-Anne and Conneau, Alexis and Chaudhary, Vishrav and Guzm{\'a}n, Francisco and Joulin, Armand and Grave, Edouard},
  booktitle = {Proceedings of the Twelfth Language Resources and Evaluation Conference},
  year      = {2020},
  pages     = {4003--4012},
  url       = {https://aclanthology.org/2020.lrec-1.494/}
}

@misc{penedo2023refinedweb,
  title        = {The {RefinedWeb} Dataset for {Falcon} {LLM}: Outperforming Curated Corpora with Web Data, and Web Data Only},
  author       = {Penedo, Guilherme and Malartic, Quentin and Hesslow, Daniel and Cojocaru, Ruxandra and Cappelli, Alessandro and Alobeidli, Hamza and Pannier, Baptiste and Almazrouei, Ebtesam and Launay, Julien},
  year         = {2023},
  howpublished = {arXiv:2306.01116},
  doi          = {10.48550/arXiv.2306.01116},
  url          = {https://arxiv.org/abs/2306.01116}
}

@misc{penedo2024fineweb,
  title        = {The {FineWeb} Datasets: Decanting the Web for the Finest Text Data at Scale},
  author       = {Penedo, Guilherme and Kydl{\'i}{\v{c}}ek, Hynek and Ben Allal, Loubna and Lozhkov, Anton and Mitchell, Margaret and Raffel, Colin and Von Werra, Leandro and Wolf, Thomas},
  year         = {2024},
  howpublished = {arXiv:2406.17557},
  doi          = {10.48550/arXiv.2406.17557},
  url          = {https://arxiv.org/abs/2406.17557}
}

@inproceedings{xue-etal-2021-mt5,
  title     = {{mT}5: A Massively Multilingual Pre-trained Text-to-Text Transformer},
  author    = {Xue, Linting and Constant, Noah and Roberts, Adam and Kale, Mihir and Al-Rfou, Rami and Siddhant, Aditya and Barua, Aditya and Raffel, Colin},
  booktitle = {Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (NAACL-HLT)},
  year      = {2021},
  url       = {https://aclanthology.org/2021.naacl-main.41/}
}

@article{Ben:Fri:18,
  author  = {Bender, Emily M. and Friedman, Batya},
  title   = {Data Statements for Natural Language Processing: Toward Mitigating System Bias and Enabling Better Science},
  journal = {Transactions of the Association for Computational Linguistics},
  volume  = {6},
  pages   = {587--604},
  year    = {2018},
  doi     = {10.1162/tacl_a_00041},
  url     = {https://doi.org/10.1162/tacl_a_00041}
}

@misc{gebru2018datasheets,
  title        = {Datasheets for Datasets},
  author       = {Gebru, Timnit and Morgenstern, Jamie and Vecchione, Briana and Vaughan, Jennifer Wortman and Wallach, Hanna and Daum{\'e} III, Hal and Crawford, Kate},
  year         = {2018},
  howpublished = {arXiv:1803.09010},
  doi          = {10.48550/arXiv.1803.09010},
  url          = {https://arxiv.org/abs/1803.09010}
}

@misc{mitchell2018modelcards,
  title        = {Model Cards for Model Reporting},
  author       = {Mitchell, Margaret and Wu, Simone and Zaldivar, Andrew and Barnes, Parker and Vasserman, Lucy and Hutchinson, Ben and Spitzer, Elena and Raji, Inioluwa Deborah and Gebru, Timnit},
  year         = {2018},
  howpublished = {arXiv:1810.03993},
  doi          = {10.48550/arXiv.1810.03993},
  url          = {https://arxiv.org/abs/1810.03993}
}

@misc{elazar2023wimbd,
  title        = {What's In My Big Data?},
  author       = {Elazar, Yanai and Bhagia, Akshita and Magnusson, Ian and Ravichander, Abhilasha and Schwenk, Dustin and Suhr, Alane and Walsh, Pete and Groeneveld, Dirk and Soldaini, Luca and Singh, Sameer and Hajishirzi, Hanna and Smith, Noah A. and Dodge, Jesse},
  year         = {2023},
  howpublished = {arXiv:2310.20707},
  doi          = {10.48550/arXiv.2310.20707},
  url          = {https://arxiv.org/abs/2310.20707}
}

@misc{liang2022helm,
  title        = {{Holistic Evaluation of Language Models}},
  author       = {Liang, Percy and Bommasani, Rishi and others},
  year         = {2022},
  howpublished = {arXiv:2211.09110},
  doi          = {10.48550/arXiv.2211.09110},
  url          = {https://arxiv.org/abs/2211.09110}
}

@misc{srivastava2022bigbench,
  title        = {Beyond the Imitation Game: Quantifying and extrapolating the capabilities of language models},
  author       = {Srivastava, Aarohi and Rastogi, Abhinav and Rao, Abhishek and others},
  year         = {2022},
  howpublished = {arXiv:2206.04615},
  doi          = {10.48550/arXiv.2206.04615},
  url          = {https://arxiv.org/abs/2206.04615}
}

@misc{hendrycks2020mmlu,
  title        = {Measuring Massive Multitask Language Understanding},
  author       = {Hendrycks, Dan and Burns, Collin and Basart, Steven and Zou, Andy and Mazeika, Mantas and Song, Dawn and Steinhardt, Jacob},
  year         = {2020},
  howpublished = {arXiv:2009.03300},
  doi          = {10.48550/arXiv.2009.03300},
  url          = {https://arxiv.org/abs/2009.03300}
}

@inproceedings{rajpurkar-etal-2016-squad,
  title     = "{SQ}u{AD}: 100,000+ Questions for Machine Comprehension of Text",
  author    = {Rajpurkar, Pranav and Zhang, Jian and Lopyrev, Konstantin and Liang, Percy},
  booktitle = {Proceedings of the 2016 Conference on Empirical Methods in Natural Language Processing},
  year      = {2016},
  month     = nov,
  address   = {Austin, Texas},
  publisher = {Association for Computational Linguistics},
  pages     = {2383--2392},
  doi       = {10.18653/v1/D16-1264},
  url       = {https://aclanthology.org/D16-1264/}
}


@inproceedings{yang-etal-2018-hotpotqa,
  title     = "{H}otpot{QA}: A Dataset for Diverse, Explainable Multi-hop Question Answering",
  author    = {Yang, Zhilin and
               Qi, Peng and
               Zhang, Saizheng and
               Bengio, Yoshua and
               Cohen, William W. and
               Salakhutdinov, Ruslan and
               Manning, Christopher D.},
  booktitle = {Proceedings of the 2018 Conference on Empirical Methods in Natural Language Processing},
  year      = {2018},
  month     = oct,
  address   = {Brussels, Belgium},
  publisher = {Association for Computational Linguistics},
  pages     = {2369--2380},
  doi       = {10.18653/v1/D18-1259},
  url       = {https://aclanthology.org/D18-1259/}
}


@book{bloom1956taxonomy,
  title     = {Taxonomy of Educational Objectives: The Classification of Educational Goals. Handbook I: Cognitive Domain},
  author    = {Bloom, Benjamin S. and Engelhart, Max D. and Furst, Edward J. and Hill, Walker H. and Krathwohl, David R.},
  year      = {1956},
  publisher = {David McKay Company, Inc.},
  address   = {New York, NY}
}


@book{anderson2001taxonomy,
  title     = {A Taxonomy for Learning, Teaching, and Assessing: {A} Revision of {Bloom's} Taxonomy of Educational Objectives},
  editor    = {Anderson, Lorin W. and Krathwohl, David R.},
  year      = {2001},
  publisher = {Longman},
  address   = {New York, NY}
}


@misc{zheng2023judging,
  title         = {Judging {LLM}-as-a-Judge with {MT}-Bench and Chatbot Arena},
  author        = {Zheng, Lianmin and Chiang, Wei-Lin and Sheng, Ying and Zhuang, Siyuan and Wu, Zhanghao and Zhuang, Yonghao and Lin, Zi and Li, Zhuohan and Li, Dacheng and Xing, Eric P. and Zhang, Hao and Gonzalez, Joseph E. and Stoica, Ion},
  year          = {2023},
  howpublished  = {arXiv preprint},
  eprint        = {2306.05685},
  archivePrefix = {arXiv},
  doi           = {10.48550/arXiv.2306.05685},
  url           = {https://arxiv.org/abs/2306.05685}
}


@inproceedings{liu-etal-2023-g-eval,
  title     = "{G}-Eval: {NLG} Evaluation using {GPT}-4 with Better Human Alignment",
  author    = {Liu, Yang and Iter, Dan and Xu, Yichong and Wang, Shuohang and Xu, Ruochen and Zhu, Chenguang},
  booktitle = {Proceedings of the 2023 Conference on Empirical Methods in Natural Language Processing},
  year      = {2023},
  month     = dec,
  address   = {Singapore},
  publisher = {Association for Computational Linguistics},
  pages     = {2511--2522},
  doi       = {10.18653/v1/2023.emnlp-main.153},
  url       = {https://aclanthology.org/2023.emnlp-main.153/}
}

@inproceedings{tsarfaty-etal-2020-spmrl,
  title     = {{SPMRL}-{SANCL} 2014 Shared Task on Parsing Morphologically Rich Languages},
  author    = {Tsarfaty, Reut and Seddah, Djam{\'e} and Goldberg, Yoav and K{\"u}bler, Sandra and Candito, Marie and Foster, Jennifer and Versley, Yannick and Rehbein, Ines and Tounsi, Lamia},
  booktitle = {Proceedings of the First Joint Workshop on Statistical Parsing of Morphologically Rich Languages and Syntactic Analysis of Non-Canonical Languages},
  year      = {2014},
  address   = {Dublin, Ireland},
  publisher = {Dublin City University},
  pages     = {103--109},
  url       = {https://aclanthology.org/W14-6111/}
}

@inproceedings{gerz-etal-2018-relation,
  title     = {On the Relation between Linguistic Typology and (Limitations of) Multilingual Language Modeling},
  author    = {Gerz, Daniela and Vuli{\'c}, Ivan and Ponti, Edoardo Maria and Reichart, Roi and Korhonen, Anna},
  booktitle = {Proceedings of the 2018 Conference on Empirical Methods in Natural Language Processing},
  year      = {2018},
  month     = oct,
  address   = {Brussels, Belgium},
  publisher = {Association for Computational Linguistics},
  pages     = {316--327},
  doi       = {10.18653/v1/D18-1029},
  url       = {https://aclanthology.org/D18-1029/}
}

@article{coltekin2023turkish,
  title     = {Resources for {Turkish} Natural Language Processing: {A} Critical Survey},
  author    = {{\c{C}}{\"o}ltekin, {\c{C}}a{\u{g}}r{\i} and Do{\u{g}}ru{\"o}z, A. Seza and {\c{C}}etino{\u{g}}lu, {\"O}zlem},
  journal   = {Language Resources and Evaluation},
  volume    = {57},
  pages     = {449--488},
  year      = {2023},
  publisher = {Springer},
  doi       = {10.1007/s10579-022-09605-4},
  url       = {https://doi.org/10.1007/s10579-022-09605-4}
}
